Structurally Diverse Sampling for Sample-Efficient Training and Comprehensive Evaluation

A growing body of research has demonstrated the inability of NLP models to generalize compositionally and has tried to alleviate it through specialized architectures, training schemes, and data augmentation, among other approaches. In this work, we study a different approach: training on instances with diverse structures. We propose a model-agnostic algorithm for subsampling such sets of instances from a labeled instance pool with structured outputs. Evaluating on both compositional template splits and traditional IID splits of 5 semantic parsing datasets of varying complexity, we show that structurally diverse training using our algorithm leads to comparable or better generalization than prior algorithms in 9 out of 10 dataset-split type pairs. In general, we find structural diversity to consistently improve sample efficiency compared to random train sets. Moreover, we show that structurally diverse sampling yields comprehensive test sets that are a lot more challenging than IID test sets. Finally, we provide two explanations for improved generalization from diverse train sets: 1) improved coverage of output substructures, and 2) a reduction in spurious correlations between these substructures.

==> 1_extended_intro.tex <==
\section{Introduction}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/substructures.png}
    \caption{An instance from the \covr{} dataset along with its abstract syntax tree (AST) and different types of substructures in it, including template, bigrams and subtrees. Note that subtrees will also include each individual node in the AST.}
    \label{fig:substructures}
\end{figure}

Systematic compositionality---expressing novel complex concepts as a systematic composition of expressions for simpler concepts---is the property underlying human languages' expressive power \cite{lake2017building,fodor1988connectionism}. However, NLP models struggle to generalize to novel composite expressions in the context of semantic parsing~\cite{lake2018scan,loula-etal-2018-rearranging,kim-linzen-2020-cogs}.

Data augmentation has been extensively explored for compositional generalization~\cite{Akyrek2021LearningTR,guo2021revisiting,wang-etal-2021-learning-synthesize,guo-etal-2020-sequence,qiu-etal-2021-csl}. However, instances in semantic parsing possess structure, such as abstract syntax trees (ASTs) of target programs (Figure \ref{fig:substructures}). Randomly selecting instances from a grammar, or even from human annotators, while ignoring similarity in their structure is likely to produce skewed distributions with spurious correlations between substructures. This \textit{task ambiguity} and \textit{underspecification} are known to cause overparameterized models to have high variance and poor generalization \cite{damour-etal-2020-underspecification,geirhos-etal-2020-shortcut-learning}.
In contrast, a structurally diverse set of instances containing a variety of different structures should better cover the combinatorial space of structures and yield more sample-efficient train sets.

Prior work on diverse sampling has shown improved sample efficiency in compositional (non-IID) splits, by
selecting instances to have diverse \emph{program templates}~\cite{oren-etal-2021-finding} or \emph{AST bigrams}~\cite{bogin2022unobserved} (see Figure~\ref{fig:substructures} for examples). However, for reasonably-sized programs, templates are very large structures, and bigrams are very small; focusing on either one of these on its own does not necessarily improve diversity across a range of differently-sized structures. Moreover, there is limited evidence of sample efficiency of diverse train sets in the IID setting and no exploration of diverse test sets.

In this study, we take a broader look at the advantages of structural diversity. We begin with the hypothesis that a diverse sample of instances that contain a variety of different substructures would both better cover the combinatorial space of structures and reduce spurious correlations between substructures compared to random instances.
A structurally diverse train set should thus be more informative about the \textit{system} underlying the instances' structures and hence improve generalization.
Similarly, a structurally diverse test with its improved coverage of structures should test for a lot more reasoning patterns than a randomly sampled IID test set and hence make for a more comprehensive evaluation.
This is analogous to how one would choose to evaluate on a test set with balanced classes even when the training data might have a considerable imbalance.

We thus propose a general, substructure and model-agnostic recipe for structurally diverse subsampling algorithms that interleaves selecting unseen substructures and instances containing those substructures and for appropriate definitions of substructures, and substructure and instance-weighting schemes, subsumes both template and bigram diversity. Experimenting with algorithms with different substructure and instance selection criteria we find improved performance from, 1) prioritizing selection of more frequent unseen substructures in the training pool, 2) using subtrees as substructures that are neither too granular (bigrams) nor too large (templates), and 3) simultaneously diversifying over both small (subtree) and larger (template) substructures.

Evaluating on template and IID splits of five semantic parsing datasets of varying complexities, we show that training on diverse train sets outperforms random train sets in 9 out 10 splits, often with 2x or more sample efficiency gains. In particular, our proposed subtree diversity algorithm is the most consistent, performing comparably or better than template and bigram diversity in 6 out of 10 splits, with both bigram and template algorithms often performing worse than random subsampling in IID splits.

We further study the efficacy of diversely sampled test sets and find that our diverse sampling algorithm indeed yields more comprehensive test sets that are more challenging than IID tests, especially when training on random train sets. Finally, comparing random and structurally diverse subsamples, we show that the latter 1) better cover the space of substructures, especially those in the long tail, and 2) have weaker spurious correlations between substructures as measured by average mutual information between pairs of substructures, confirming our hypotheses and explaining their benefits in training and evaluation.

We hope that our results demonstrating the importance of structural diversity will encourage future research on better structurally diverse sampling algorithms as well as their use to guide train and test set construction. The algorithms in this work are applicable whenever a large pool of possible output programs is available. One such setting is that of prototyping a semantic parser in a zero-data setting where a pool of outputs can be sampled from a grammar and mapped to canonical utterances that can be paraphrased for linguistic variation either manually or automatically \cite{wang-etal-2015-building,herzig-berant-2019-dont,campagna-etal-2020-zero,yin-etal-2022-ingredients}. Another scenario is that of selecting instances for in-context or few-shot learning \cite{brown-etal-2020-fewshot}. Finally, our results indicate that the failure of NLP models on compositional generalization may be due in part to the lack of diversity in them, suggesting the need to create more diverse benchmarks.


==> 4_coverage.tex <==
\section{Sample Analysis}\label{sec:coverage}

In \S\ref{sec:setup} we hypothesized that structurally diverse sampling has two benefits over random sampling: (1) it improves coverage of the space of substructures, and (2) it reduces spurious correlations. We now attempt to verify these hypotheses. As in \S\ref{sec:setup}, we assume access to a pool of instances $D_{pool} = \{e_i\}_{i=1}^n$. However, we now treat each instance $e_i$ as a set of substructures contained in it, i.e. $e_i \subset C$. Unless otherwise specified, in this section, the substructures under consideration will be subtrees.
We also define the frequency of a subtree, $s$, in a set of instances $A$ as $F_{A}(s) = |\{s \in e: e \in A\}|$ where $|.|$ is set cardinality operator. The frequency of a pair of substructures, can analogously be defined as $s_i, s_j$ as $F_{A}(s_i, s_j) = |\{s_i, s_j \in e: e \in A\}|$. We additionally define $rank(s)$ as the mapping of $s$ to its position in a list of all substructures in $A$ sorted in descending order of frequency with equally frequent substructures ordered arbitrarily.

\subsection{Improved Coverage of the Long tail}\label{sec:coverage}

Figure \ref{fig:} compares the number of unique subtrees of a given rank in the pool as well as in samples of same size obtained using random sampling and the \subt{} algorithm.
Two things are evident, first that \subt{} subsamples pack a lot more unique subtrees than random subsamples, and second, this increase in the number of subtrees comes largely from sampling the less frequent subtrees. Together these observations demonstrate that structurally diverse sampling improves coverage of substructures, especially those in the long tail.

App. \ref{app:coverage} contains additional analyses of improved coverage enabled by diverse sampling. Two findings are particularly interesting. First, as Figure \ref{fig:} shows, diverse sampling also better matches the distribution of subtrees in the pool. And second, although \subt{} algorithm only takes into consideration subtrees in output programs, it also leads to a similar improvement in coverage of output program templates as well as of input utterances. This is shown in Figures \ref{fig:}, \ref{fig:}, and \ref{fig:} which replicate the above analysis for templates derived from output programs, and unigrams and bigrams derived from input utterances.


\subsection{Weakened Spurious Correlations}\label{sec:correlation}

Now we attempt to verify whether using a diverse set of instances also reduces the spurious correlations between substructures. We begin by defining a measure correlations between substructures in a set of instances $D$ as the sum of pairwise mutual information (MI) between them, normalized to take into account the larger number of distinct substructures in diverse subsamples. Formally, as earlier, we view each instance as a bag of substructures, specifically subtrees of size $\leq d = 4$ with $S = {s_1, \ldots, s_m}$ as the set of all subtrees. We define an indicator random variable $I_s$ for each subtree $s$ that is 1 if $s$ is present in a random instance, 0 otherwise. MI between two subtrees, $s_i$ and $s_j$ is then defined as,

\begin{equation}
    \operatorname{MI}[s_i, s_j] = -\sum\limits_{I_{s_i}, I_{s_j}} \tilde{p}(I_{s_i}, I_{s_j}) \log \frac{\tilde{p}(I_{s_i}, I_{s_j})}{\tilde{p}(I_{s_i})\tilde{p}(I_{s_j})}
\end{equation}

where $\tilde{p}(I_s=1)$ is the empirical probability of $s$ occurring in an instance and $\tilde{p}(I_{s_i}=1, I_{s_j}=1)$ is the empirical probability that $s_i$ and $s_j$ co-occur in an instance, i.e.

\begin{align}
    \tilde{p}(s=1) &= \frac{|\{s \in e: e \in D\}|}{|D|} \\
    \tilde{p}(s_i=1, s_j=1) &= \frac{|\{s_i, s_j \in e: e \in D\}|}{|D|}
\end{align}

Other probabilities are defined analogously. Our measure of correlations is then the average mutual information (AMI) across all subtree pairs.

\begin{equation}
    \operatorname{AMI}(D) = \frac{1}{|S|^2}\sum\limits_{i, j} \operatorname{MI}[s_i, s_j]
\end{equation}

\input{tables/corr}

Finally, Figure \ref{fig:diverse-corr} compares the AMI of \subt{} and random subsamples of varying sizes taken form $D_{pool}$ for each dataset showing that diverse subsamples have lower correlations.

==> 7_lexical.tex <==
\section{Lexical Diversity}
\label{sec:lexical}

Given the success of diversity in improving generalization, we now investigate whether it can also improve performance on existing compositional generalization benchmarks. 

\subsection{Benchmarks}
\label{sec:lex-benchmarks}
We experiment with two benchmarks SCAN \cite{lake2018scan} and COGS \cite{kim-linzen-2020-cogs}. 

\tightparagraph{\textbf{SCAN}} is a synthetic semantic parsing benchmark consisting of simple compositional commands paired with action sequences. Each command may contain verbs (\textit{walk, run, look} and \textit{jump}), directions (\textit{left} or \textit{right}) along with some modifiers for manner and repetition of actions and conjunction. We show an examples instance in Table \ref{tab:ds-samples} and refer the reader to \cite{lake2018scan} for more details of the dataset. We experiment with the \textsc{AddJump} split from the benchmark which tests for compositional generalization by holding out all but the most primitive instances with the verb \textit{jump} i.e. \textit{jump} $\rightarrow$ JUMP. Standard seq2seq models completely fail on this split, as it requires them model to generalize from the other verbs to \textit{jump} i.e. understand the verb independent of its context.

\tightparagraph{\textbf{COGS}} is also a semantic parsing benchmark consisting of a variety of English sentence constructions with 400 nouns and 80 verbs of different types. These are generated using a PCFG and paired with a logical form representing the semantic roles of verbs and nouns in the sentence. The benchmark consists of multiple systematic gaps that require compositional generalization. These include new combinations of familiar structures (eg. \textit{active} $\rightarrow$ \textit{passive}, deeper PP-recursion etc.) or new combinations of familiar primitives and structures (eg. \textit{subject} $\rightarrow$ \textit{object}). We include an example instance from COGS in Table \ref{tab:ds-samples} and refer to \cite{kim-linzen-2020-cogs} for details of the benchmark.

\subsection{Setup}
\label{sec:lex-setup}
Since increasing the structural diversity in \scan{} and \cogs{} would change the systematic gaps they test against, in these experiments, we 
increase diversity differently. We conjecture that the compositional generalization failures on these benchmarks may be due in part to limited lexical diversity, i.e. number of nouns and verbs, which makes it harder for models to decorrelate those words meaning from the structure of the context. Taking advantage of the availability of the generation process of these datasets, we thus experiment with increasing their lexical diversity. This has been previously shown to improve performance on the \textsc{AddJump} split by \citet{kagitha}, however, they do not control for the increase in training set size with more verbs hence its not clear whether the improved generalization was due to increased diversity or merely more data. We thus perform our experiments keeping the size of the train sets and systematic gaps between the train and test sets fixed.

\subsection{Model and Training}
\label{sec:lex-training}


\subsection{Results}
\label{sec:lexical-results}

Fig. \ref{fig:scan-diverse} and \ref{fig:cogs-diverse} show the results of varying lexical diversity on SCAN and COGS. It is evident that increasing lexical diversity improves generalization showing that diversity helps improve generalization.



==> 7_lexical_orig.tex <==
\section{Lexical Diversity}
\label{sec:lexical}
\sg{decide whether to keep this}

Given the success of diversity in improving generalization, we now investigate whether it can also improve performance on existing compositional generalization benchmarks. 

\subsection{Benchmarks}
We experiment with two benchmarks, SCAN \cite{lake2018scan} and COGS \cite{kim-linzen-2020-cogs}. 

\tightparagraph{SCAN} is a synthetic semantic parsing benchmark consisting of simple compositional commands paired with action sequences. Each command may contain a verb eg. \textit{walk, run, look} and \textit{jump}, a direction i.e. \textit{left} or \textit{right} along with some modifiers for nature and repetition of primitive actions and conjunction. We show an examples instance in Table \ref{tab:ds-samples} and refer the reader to \cite{lake2018scan} for more details of the dataset. The benchmark tests for compositional generalization by training only on the most primitive instance with \textit{jump} i.e. \textit{jump} $\rightarrow$ JUMP along with all instances with the other verbs and then testing on complex instances with \textit{jump}. Standard seq2seq models completely fail on this split, termed the \textsc{AddJump} split, as it requires them model to generalize from the other verbs to \textit{jump} i.e. understand the verb independent of its context.


We experiment with two benchmarks, SCAN \cite{lake2018scan} and COGS \cite{kim-linzen-2020-cogs}. 
Since the output formalism in these two is not amenable to structural 

We begin by motivating the utility of diversity through proof-of-concept experiments showing that merely increasing lexical diversity i.e. the number of open class words such as nouns and verbs is sufficient to improve performance on SCAN \cite{lake2018scan} and COGS \cite{kim-linzen-2020-cogs} benchmarks.

\subsection{SCAN}
\label{sec:scan}

SCAN is a synthetic semantic parsing benchmark consisting of simple compositional commands paired with action sequences. Each command may contain a verb eg. \textit{walk, run, look} and \textit{jump}, a direction i.e. \textit{left} or \textit{right} along with some modifiers for nature and repetition of primitive actions and conjunction. We show an examples instance in Table \ref{tab:ds-samples} and refer the reader to \cite{lake2018scan} for more details of the dataset. The benchmark tests for compositional generalization by training only on the most primitive instance with \textit{jump} i.e. \textit{jump} $\rightarrow$ JUMP along with all instances with the other verbs and then testing on complex instances with \textit{jump}. Standard seq2seq models completely fail on this split, termed the \textsc{AddJump} split, as it requires them model to generalize from the other verbs to \textit{jump} i.e. understand the verb independent of its context.

We conjecture that this failure may be due not just to the models' inability to generalize compositionally but also because three verbs may be insufficient for the model to learn to de-correlate the verb from its context. We thus experiment with increasing the number of verbs that the model sees during training. While this has been shown to improve performance on \textsc{AddJump} split by \cite{kagitha}, however they do not control for the increase in training set size with more verbs hence its not clear whether the improved generalization was due to increased diversity or merely more data. We thus perform the same experiment with varying lexical diversity in terms of number of verbs in the \textit{AddJump} but with the same training set size. Additionally we also perform the same experiment with a \textsc{Switch} split wherein the model is shown half the verbs with repetition \textit{twice} and half with \textit{thrice} and is required to generalize to commands with the repetition switched.


\subsection{COGS}
\label{sec:cogs}

COGS \cite{kim-linzen-2020-cogs} is a compositional generalization benchmark consisting of a veriety of english sentence constructions generated using a PCFG and paired with semantic interpretation (semantic parsing). The compositional test set in the benchmark consists of multiple systematic gaps that require compositional generalization. These include new combinations of familiar structures (eg. \textit{active} $\rightarrow$ \textit{passive}, deeper PP-recursion etc.) or new combinations of familiar primitives and structures (eg. \textit{subject} $\rightarrow$ \textit{object}). We include an example instance from COGS in Table \ref{tab:ds-samples} and refer to \cite{kim-linzen-2020-cogs} for details of the benchmark.

COGS consists of sentences generated using 400 nouns of and 80 different types of nouns and verbs respectively. We again experiment with varying the lexical diversity i.e. the number of nouns and verbs keeping the size of the training set and the systematic gaps with respect to the compositional test set fixed.


\subsection{Results}
\label{sec:lexical-results}

Fig. \ref{fig:scan-diverse} and \ref{fig:cogs-diverse} show the results of varying lexical diversity on SCAN and COGS. It is evident that increasing lexical diversity improves generalization showing that diversity helps improve generalization.


